Context Generation from Formal Specifications for C Analysis Tools

Analysis tools like abstract interpreters, symbolic execution tools and testing tools usually require a proper context to give useful results when analyzing a particular function. Such a context initializes the function parameters and global variables to comply with function requirements. However it may be error-prone to write it by hand: the handwritten context might contain bugs or not match the intended specification. A more robust approach is to specify the context in a dedicated specification language, and hold the analysis tools to support it properly. This may mean to put significant development efforts for enhancing the tools, something that is often not feasible if ever possible. This paper presents a way to systematically generate such a context from a formal specification of a C function. This is applied to a subset of the ACSL specification language in order to generate suitable contexts for the abstract interpretation-based value analysis plug-ins of Frama-C, a framework for analysis of code written in C. The idea here presented has been implemented in a new Frama-C plug-in which is currently in use in an operational industrial setting.

==> constraints_grammar.tex <==
\begin{figure*}[htbp]
\[\arraycolsep=5pt
\begin{array}{lrll}
  % Constraints
  \textnormal{State Constraints} & \cstrone ::=
  & \srangeone \oplus \{ \rtestone \} & \textnormal{symbolic range with set of runtime tests}
  \\[2mm]

  \textnormal{Tests} & \rtestone ::=
  & \test{\termone~\kw{cop}~\termone}  & \textnormal{runtime conditional with
    $\kw{cop}\in\{\equiv,\,\leq\}$}
  % & \mid & \nalias{\memone} & \textnormal{no-aliasing with
  %   $\memone$}\\
  % & \mid & \undef & \textnormal{undefinedness}
\end{array}
\]
\caption{Grammar of state constraints and tests.}
\label{fig:syntax_constraints}
\end{figure*}

==> contract_syntax.tex <==
\begin{figure*}[htbp]
\[
\begin{array}{lrl}
  \textnormal{Function Contracts} & contract ::= &
  (behavior)^*~(completeness\_clause)^* \\
  & \mid & requires\_clause
  \\[2mm]
  \textnormal{Preconditions} & requires\_clause ::= & \kw{requires}~\predone;
%  & \mid & \kw{requires}~A \Rightarrow P; & P \textnormal{ under assumption } A
  \\[2mm]
%  \textnormal{[Assumptions]} & A ::= & \kw{true} & \\
%  & \mid & P & 
%  \\[2mm]
  \textnormal{Named Behaviors} & behavior ::= & \kw{behavior}~\ name:
  requires\_clause
  \\[2mm]
  \textnormal{Behavior Properties} & completeness\_clause ::= & \kw{complete
    behaviors}~ (name~ (,~ name)^*)^?\\
  & \mid & \kw{disjoint behaviors}~ (name~ (,~ name)^*)^?
\end{array}
\]
\caption{\acsl contract syntax (\textit{fragment}).}\label{fig:syntax_contract}
\end{figure*}


==> sexprs_grammar.tex <==
\begin{figure*}[htbp]
\[\arraycolsep=5pt
\begin{array}{lrll}
  % Symbolic Expressions
  \textnormal{Symbolic Expressions} & \sexpone ::=
  & \intone & \textnormal{integer constant ($\intone\in\intset$)} \\
  & \mid & \sidone & \textnormal{symbolic lvalue} \\
  %& \mid & \& \sidone & \textnormal{address} \\
  & \mid & \sexpone~\kw{bop}~\sexpone & \textnormal{arithmetic operation
    ($\kw{bop}\in\{\kw{+},\,\kw{-},\,\times,\,\kw{/},\,\kw{\%}\}$)}
\\
  & \mid & \semax{\sexpone}{\sexpone} & \textnormal{largest expression operation} \\
  & \mid & \semin{\sexpone}{\sexpone} & \textnormal{smallest expression operation}
  \\[2mm]
  
  % Identifiers
  \textnormal{Symbolic Lvalues} & \sidone ::= & \cvarone & \textnormal{\C variable} \\
  & \mid & \star\sexpone & \textnormal{dereference}
\end{array}
\]
\caption{Symbolic expressions.}
\label{fig:syntax_sexp}
\end{figure*}


==> soundness.tex <==
This appendix is devoted to proving Theorem~\ref{thm:soundness}. For reasons of
clarity, we actually reformulate the result in terms of two lemmas that, once
combined, prove the theorem. Note that the following formulations mention a
dependency graph $\mathcal{G}$, which was not the case in the actual statement
of Theorem~\ref{thm:soundness}. This is because we did not provide a
formalization for such graph, and the fact that one needs $\mathcal{G}$ only
when detailing proofs.

The following lemma proves that the system of simplification rules terminates.

\begin{lemma}
\label{lemma:termination}
For all conjunctive clause $\predone$, either $\emptyset, \emptyset \vdash \predone
\Rightarrow \mem, \mathcal{G}$ or it fails.
\end{lemma}

\proof[Sketch] Only finite derivations are possible: rules on literals
\kw{defined} are inductively defined on structurally smaller literals (on
smaller terms), and the others reduce to this latter. The only delicate point
concerns aliasing and, in particular, rule \textsc{Range-2}. Indeed, if
$\predone$ is a conjunctive clause that provides mutually defined predicates
(\eg{} by requiring $\bigwedge_{i=1}^j \lvalone_i\equiv
\lvalone_{(i+1)\kw{\%}j}$), then \textsc{Range-2} may cause a circular, hence
infinite, derivation. This is not the case since circular dependencies between
left-values are prevented, by construction, by the use of the dependency graph
$\mathcal{G}$. \qed

\vspace{.2cm} The following lemma proves that the system of simplification rules
provides correct results with respect to given preconditions.

\begin{lemma}
\label{lemma:correctness}
For all conjunctive clause $\predone$, $\mem \vdash \predone
\Rightarrow \mem'$ implies $\mem' \models \predone$.
\end{lemma}

\proof[Sketch] Reasoning by induction on the derivation $\mem \vdash \predone
\Rightarrow \mem'$, and by considering the form of $\predone$. If the last rule
is \textsc{And}, then $\predone$ is a conjunction $\bigwedge_i \predone_i$. The
result follows by trivially composing the results of the induction hypothesis on
each $\predone_i$. Hence, let us now consider rules in
Figure~\ref{fig:predicates2constraints} for positive literals. We do not
consider rules for negative literals as they just check consistency, which we
get as hypothesis of having a derivation.

The cases that assign initial ranges for predicates \kw{defined}, \ie{} rules
\textsc{Variable} and \textsc{Dereference}, trivially hold. There is nothing to
prove for rule \textsc{Idempotence}.

Let us now suppose $\predone$ of the form
$\defpred{\lvalone~\kw{++}\range{\termone_1}{\termone_2}}$ and rule
\textsc{Range-1} is used for deriving $\mem \vdash
\defpred{\lvalone~\kw{++}\range{\termone_1}{\termone_2}}\Rightarrow \mem''$. By
the induction hypothesis% on $\defpred{\lvalone}$
, there is $\mem'$ such that $\mem' \models \defpred{\lvalone}\wedge
0\leq\termone_1\leq\termone_2$. Then, since the range of $\lvalone$ in $\mem''$
is computed as $\proj{1}{\mem'\left(\lvalone\right)}\sqcup \ival{0}{\termone_2}$
and
$\ival{\termone_1}{\termone_2}\subseteq\ival{0}{\termone_2}\subseteq\proj{1}{\mem'\left(\lvalone\right)}\sqcup
\ival{0}{\termone_2}$, it follows $\mem''\models \predone$. In the case
\textsc{Range-2} has been used, $\lvalone$ points to $\lvalone'+\termone_3$,
\ie{}, $\lvalone\equiv \lvalone'+\termone_3$. The result follows by the
induction hypothesis and the fact that $\ival{\termone_1}{\termone_2}\subseteq
\ival{\semin{\termone_1}{\termone_3}}{\semax{\termone_2}{\termone_3}}$.

Let us now consider the cases \textsc{Cmp-1} and \textsc{Cmp-2}. The former case
holds for similar reasons as \textsc{Range-1}, \ie{}, by observing that the
range value of $\lvalone$ is safely computed in terms of $\sqcap$. The latter
case holds by the definition of runtime check.

If rule \textsc{Memory-Eq} has been used, then $\predone$ is, without loss of
generality, of the form $\lvalone_1 \equiv \lvalone_2+\termone$. By the
induction hypothesis, there is $\mem'$ such that $\mem'\models
\defpred{\lvalone_1} \wedge \defpred{\lvalone_2+\termone}$. The result follows
by the fact that $\lvalone_1$ is imposed to point to $\lvalone_2+\termone$ as
required, and that $\proj{1}{\mem'\left(\lvalone_1\right)} \sqsubseteq
\proj{1}{\mem'\left(\lvalone_2\right)}$, \ie{} no memory access via $\lvalone_1$
overflows the memory region defined by $\lvalone_2$. \qed

\vspace{0.2cm} It is easy to see that Theorem~\ref{thm:soundness} follows from
Lemmas~\ref{lemma:termination} and~\ref{lemma:correctness}.


==> terms2sexprs.tex <==
\begin{figure*}[htbp]
% Left-Values
\[
\inferrule[TERM-VAR$_{1}$]{\envof{\cvarone}=\vid{\cvarone}}{\termtosid{\env}{\cvarone}{\vid{\cvarone}, \env}}
\qquad\qquad
\inferrule[TERM-VAR$_{2}$]{\cvarone\not\in\env\\ \env'=\envupdate{\cvarone}{\vid{\cvarone}}}{\termtosid{\env}{\cvarone}{\vid{\cvarone}, \env'}}
\qquad\qquad
\inferrule[TERM-MEM$_{\star}$]{\termtosid{\env}{\memone}{\sidone', \env'}\\ \sidone=\memacstwo{\sidone'}}{\termtosid{\env}{\memacstwo{\memone}}{\sidone, \env'}}
\]
% Memory Values
\[
% \inferrule[$MEM_{LV}$]{\termtosid{\env}{\lvalone}{\sidone, \env'}}{\termtosid{\env}{\lvalone}{\sidone, \env'}}
% \qquad\qquad
\inferrule[TERM-MEM$_{\&}$]{\termtosid{\env}{\lvalone}{\sidone', \env'}\\
  \sidone = \&\sidone'}{\termtosid{\env}{\&\lvalone}{\sidone, \env'}}\qquad\qquad
% \]
% \[
\inferrule[TERM-MEM$_{\kw{++}}$]{\termtosid{\env}{\memone}{\sidone', \env'}\\ \termtosid{\env'}{\termone}{\sexpone, \env''}\\ \sidone=\sidone'~\kw{++}~\sexpone}{\termtosid{\env}{\memone~\kw{++}~\termone}{\sidone, \env''}}
\]
% Integer terms
\[
\inferrule[TERM-NUM]{}{\termtosid{\env}{\intone}{\intone, \env}}
\qquad\qquad
\inferrule[TERM-${\kw{bop}}$]{\termtosid{\env}{\termone_1}{\sexpone_1, \env'} \qquad \termtosid{\env'}{\termone_2}{\sexpone_2, \env''}\\ \sexpone = \sexpone_1~\kw{bop}~\sexpone_2 % \\ \kw{bop}\in\{~\kw{+}~,~\kw{-}~,~\times~,~\kw{/}~,~\kw{\%}~\}
}{\termtosid{\env}{\termone_1~\kw{bop}~\termone_2}{\sexpone, \env''}}
\]
\caption{Translation of \acsl terms into symbolic expressions.}\label{fig:identifiers}
\end{figure*}
